Covert Planning against Imperfect Observers

Covert planning refers to a class of constrained planning problems where an agent aims to accomplish a task with minimal information leaked to a passive observer to avoid detection. However, existing methods of covert planning often consider deterministic environments or do not exploit the observer's imperfect information. This paper studies how covert planning can leverage the coupling of stochastic dynamics and the observer's imperfect observation to achieve optimal task performance without being detected. Specifically, we employ a Markov decision process to model the interaction between the agent and its stochastic environment, and a partial observation function to capture the leaked information to a passive observer. Assuming the observer employs hypothesis testing to detect if the observation deviates from a nominal policy, the covert planning agent aims to maximize the total discounted reward while keeping the probability of being detected as an adversary below a given threshold. We prove that finite-memory policies are more powerful than Markovian policies in covert planning. Then, we develop a primal-dual proximal policy gradient method with a two-time-scale update to compute a (locally) optimal covert policy. We demonstrate the effectiveness of our methods using a stochastic gridworld example. Our experimental results illustrate that the proposed method computes a policy that maximizes the adversary's expected reward without violating the detection constraint, and empirically demonstrates how the environmental noises can influence the performance of the covert policies.

==> almost-sure-case.tex <==

 \subsection{Detection-Aware Policy Gradient: Almost-Sure Case}
\begin{definition}
    An almost-sure no-detection and optimal strategy parameter $\theta$ is the solution to the following problem.
\begin{alignat}{2}
    & \optmax_\theta && V (s_0, \theta) \label{eq:almost-sure-deception}
\\
 & \optsts &&   \log\frac{P(y;M_\theta)}{P( y ;  M_0)} \le \epsilon, \forall y \in \{ \mathcal{Y} \mid P(y|M_\theta)>0\}
\end{alignat}
where $M_\theta$ is the \ac{hmm} induced by the policy $\pi_\theta$ from the \ac{mdp} $M$ and the observation function $\obs$.
\end{definition}
In other words, no matter which observation is generated, the opponent cannot reject the null hypothesis   given that observation. Under this constraint, the goal is to compute a policy $\pi$ that maximize the total discounted reward given the reward function $R : S\times A\rightarrow \reals$.

However, in some cases, it maybe infeasible to require no-detection with probability one. We can relax such a constraint to allow detection to occur with a small probability.



To solve the optimization problem \ref{eq:almost-sure-deception}, it is noted that the number of constraints grows with the number of observations in the hidden Markov model. In this subsection we propose a   gradient-based method to find an approximate-optimal solution to \ref{eq:almost-sure-deception}.

Our approach is based on randomized optimization. First, let  a continuous function $B: \reals \rightarrow \reals_{+}$ be defined with support equal to $[0, \infty)$. One such function is $B(x) = \max\{x,0\}$.   Using randomized optimization~\cite{tadic2006randomized}, an equivalent representation of \eqref{eq:almost-sure-deception} is:
\begin{align}
\label{eq:randomized-opt}
    &\max_\pi V (s_0, \pi)\\
   &  \text{subject to: } \\
   &   \Expect_{\pi}\left[  B (\log\frac{P(y|M^\pi)}{P( y \mid M_0)} - \epsilon)\right] =0
\end{align}
where the expectation is taken with respect to the distributions over observations in the \ac{hmm} $M^\pi$. 

For this constrained optimization problem with an equality constraint, we consider the \emph{quadratic penalty method}. First, we replace the policy  with the policy function parameter $\theta$. Let $\pi_\theta$ be the policy function with parameter $\theta$. 
For example, the parameter $\theta$ may corresponds to the parameters in the neural network approximation of the policy function. The Markov chain  induced by policy $\pi_\theta$ is rewritten as $M_\theta$ and the expectation  over observation sequences is expressed equivalently as $\Expect_\theta$. 
For notational convenience, we denote $\Expect_{\theta}  \left[  B (\log\frac{P(y|M_\theta)}{P(y \mid M_0)}- \epsilon)\right]$    by a function $\Expect_{y \sim \dist{\theta}} h(y)$ where $ h(y) =\left[  B (\log\frac{P(y|M_\theta)}{P(y \mid M_0)}- \epsilon)\right]$.
 
Next, we define the augmented Lagrangian: For any constant $c$, the augmented Lagrangian function is defined by
\[
L_c(\theta,  u) = V(s_0, \theta) + u    \Expect_{y \sim \dist{\theta}} h(y) + \frac{1}{2} c  \left(\Expect_{y \sim \dist{\theta}} h(y)\right)^2 
\]
where  $V(s_0, \theta) = V(s_0, \pi_\theta)$ and $c$ is the penalty parameter and $u$ is the multiplier. Both $u$ and $c$ are scalars.


The quadratic penalty method is to solve a sequence of problems of the following form 
$$\mbox{maximize}_\theta L_{c_k}(\theta, u_k),$$
where  $\theta_k$ is the optimal solution from the $k$-th iteration,  $\{u_k\}$ is a bounded sequence in $\real$ and $\{c_k\}$ is a penalty parameter sequence satisfying 
$$
 c_{k+1} \le c_k \le 0, \quad \forall k, c_k \rightarrow - \infty.
$$

When $\mu_k$ is bounded and $c_k$ unbounded from below, the term $$ u_k    \Expect_{y \sim \dist{\theta}} h(y) + \frac{1}{2} c_k  \left(\Expect_{y \sim \dist{\theta}} h(y)\right)^2 $$  added to the objective function can approach $-\infty$ if the constraint is not satisfied. Thus, to maximize $L_{c_k}(\theta,u_k)$ recovers the original constrained optimization.



\subsection{Proximal Point-Based Policy Gradient Method with Almost-Sure Intention Deception}

We can perform gradient-based optimization to solve the sequence of optimization problems. Let $k$ be the step for outer-loop iteration and $i$ be the step for the inner-loop iteration. 
Initialize $\theta_0$ and $i=0$. At the iteration $i+1$, 
\[
\theta_{i+1} = \arg\max_\theta L_{c_k}(\theta,   u_k)  
\]  
To compute this update in the policy parameter, we can employ stochastic optimization approach.  However, because the objective function $L_{c_k}(\theta,    u_k)  $ contains a distribution that depends on the decision variable $\theta$, the distribution shift can affect the stability of the stochastic optimization algorithm that rely on the sampling. To mitigate this issue, we adopt a variant of proximal point method by adding a constraint on  the distance between a policy before and after an update. 

\begin{equation}
\label{eq:inner-iter}    
\theta_{i+1} =\theta_i + \nabla_\theta \left( L_{c_k}(\theta,     u_k) -\beta_i D_{KL}(\pi_{\theta}|| \pi_{\theta_i})\right) \end{equation}
where $D_{KL}(\pi_{\theta}|| \pi_{\theta_i}) $ is the KL-divergence between the policy $\pi_\theta $ and $\pi_{\theta_i}$.  

\todo[inline]{Add Explicit expression}
\todo[inline]{Add the gradient computation}
The gradient term consists of three components: The first component is the policy gradient with respect to improving the value function; the second component is the policy gradient with respect to the penalty term associated with the constraint; the last component is the policy gradient with respect to the KL-divergence between the current policy and the updated policy. It is observed that the summation of the first term and the second term is exactly the gradient used by proximal policy optimization. 

For completeness, the equations are included to compute the proximal policy gradient:

\begin{equation}
\label{eq:prox-gradient} 
todo
\end{equation}
\todo[inline]{to complete}
The second term is computed as follows.
  \begin{align}     \label{eq:gradient_obs}
 & \nabla_\theta \left( u_k  \Expect_{y \sim \dist{\theta}} h(y) + \frac{1}{2} c_k  \left(\Expect_{y \sim \dist{\theta}} h(y)\right)^2 \right)\\
  & = \left( u_k   + c_k \Expect_{y \sim \dist{\theta}} h(y) \right) \cdot \nabla_\theta\Expect_{y \sim \dist{\theta}} h(y)
\end{align}
Next, we show how to approximate the gradient $\nabla_\theta\Expect_{y \sim \dist{\theta}} h(y)$ using sampled trajectories.
\[
\nabla_\theta\Expect_{y \sim \dist{\theta}} h(y) 
 = \sum_{y}   P(y|M^\pi) \left[  B (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\right] 
 \]
Based on the stochastic gradient descent, we fix the sampling distribution to obtain an inexact gradient:
\begin{align*}
& \nabla_\theta \sum_{y}   P(y|M_\theta) \left[  B (\log\frac{P(y|M_\theta)}{P(y \mid M_0)} - \epsilon)\right]\\
  = &\nabla_\theta  \sum_{y \in \textcolor{blue}{U}}   P(y|M_\theta) (\log\frac{P(y|M_\theta )}{P(y \mid M_0)} - \epsilon)\\
  \approx  &   \sum_{y \in \textcolor{blue}{U}}   P(y|M_\theta) \nabla_\theta (\log\frac{P(y|M_\theta)}{P(y \mid M_0)} - \epsilon) \quad \text{--- inexact gradient } \\
   = &   \sum_{y \in \textcolor{blue}{U}}   P(y|M_\theta)  \nabla_\theta  \log P(y|M_\theta)\\
   = & \sum_{y \in \textcolor{blue}{U}}  \nabla_\theta P(y|M_\theta)\\
   = & \sum_{y \in \textcolor{blue}{U}}  \nabla_\theta \left( \sum_{y \in \plays(M_\theta)} P(y,y)P(y|M_\theta )\right) \quad \text{--- law of total probability} \\
   = &  \sum_{y \in \textcolor{blue}{U}}   \sum_{y \in \plays(M_\theta)} P(y|y)P(y|M_\theta) \nabla_\theta P(y|M_\theta)\\
   = & \sum_{y \in \textcolor{blue}{U}}  \sum_{y \in \plays(M_\theta)} P(y,y|M_\theta) \nabla_\theta P(y|M_\theta)\\
 \approx &    \sum_{y_i \in \textcolor{magenta}{\overline U}}  \mathbf{1}(y_i=y, y_i=y) \frac{\partial \log  P(y_i | M^{\theta})}{\partial \theta}, \quad \text{--- sample approximation}
        \end{align*} 

\cs{I suggest using a different symbol instead of $y$ here. There are two $y$s in the calculation. One $y \in U$ and another $y \in \plays(M_\theta)$. It's very confusing.}
where $U$ is a set of observations that violate the detection constraint and $\bar U = \{(y_i,y_i)\mid 0\le i \le \abs{\bar U} \}$ is a set of pairs of sampled observation sequences and state sequences from the hidden Markov model $M_\theta$.
\jf{This gradient computation maybe removed to the Appendix.}

The term $\frac{\partial \log  P(y_i | M^{\theta})}{\partial \theta}$ can be computed as follows.
\begin{equation*}
	\log P(y | M^{\theta}) = \log \prod_{t=0}^{\abs{y}} P(s_t, a_t, s_{t+1})\pi(s_t, a_t) = \sum_{t=0}^{\abs{y}} \log P(s_t, a_t, s_{t+1}) + \log \pi_\theta(s_t, a_t)
\end{equation*}
\cs{I think the calculation of $\log P(y | M^{\theta})$ has some problems. It's the sequence of observations. The calculation here will end up with the probability of the trajectory $x = s_0 a_0 s_1 \dots$. Not the observation sequence. It should contain the observation function.}

Thus, $\frac{\partial \log P(y | M^{\pi})}{\partial \pi} = \frac{\partial \sum_{t} (\log P(s_t, a_t, s_{t+1}) + \log \pi(s_t, a_t))}{\partial \pi} = \sum_{t}\frac{\partial \pi(s_t, a_t)}{\partial \pi}\frac{1}{\pi(s_t, a_t)}$. 

\cs{It should be $\frac{\partial \log P(y | M^{\theta})}{\partial \theta}$, right? }

\todo[inline]{Adding the algorithm}

When the inner-loop converges (or the target objective function values change below a given threshold before and after an update), we update the multiplier $u_k$ and the penalty parameter $c_k$ for the outer-loop and repeat until both inner and outer loop converges given the stopping criteria.

The multiplier $u_k$ is updated using the following rule:
\begin{equation}
\label{eq:update-multiplier}
\end{equation}

And the penalty parameter $c_k$ is updated using the following rule:


==> archieved/archieved-divergence.tex <==

\newpage
\section{minimizing KL divergence case}
If, instead of solving \eqref{eq:deception-planning}, we consider the problem of maximizing the reward while ensuring the KL divergence is below a given threshold, as specified in \eqref{eq:kl-constrained}. 

For this problem, we consider the planning in the state space augmented with the observations. A state $z =(s,y)$ for $s$ is the current state and $y$ is the past observations.
The observation-augmented planning problem is an \ac{mdp} $\mathcal{M} = (Z, A, P, z_0, R)$.


Let's define the following distance between the trajectory distributions introduced by $\pi_1$ and $\pi_2$. We name this distance as \emph{the divergence between average state-observation distributions.}

\begin{equation}
    D_f(m_1(z)P(y| z,\mathcal{M}_1) \parallel m_2(z)P(y| z, \mathcal{M}_2) )
= \sum_{z\in Z, o\in O}  m_1(z)P(o| z,\mathcal{M}_1) f(\frac{m_1(z)P(o| z,\mathcal{M}_1)}{m_2(z)P(o| z, \mathcal{M}_2) })
\end{equation}
where $f$ can be any function in $f$-divergence, $m_i$ is the occupancy measure induced by $\pi_i$ in the \ac{mdp} $\mathcal{M}$ and $P(o| z,\mathcal{M}_i) = \sum_{z'} P(z,a,z')\pi_i(z,a)O(z',o)$ is the probability of receiving observation $o$ given the state $z$ and policy $\pi_i$.

The following important result can help to formulate the optimization problem: (if we can prove it. The paper shows a case with complete observation: )

\begin{theorem}
Given two policies $\pi_1$ and $\pi_2$ in \ac{mdp} $\cal M$, the $f$-divergence between trajectory distribution is lower bounded by $f$-divergence between average state-observation distribution.
$$
D_f(\obs(M_1)\parallel \obs(M_2)) \ge  D_f(m_1(z)P(y| z,\mathcal{M}_1) \parallel m_2(z)P(y| z, \mathcal{M}_2) )
$$
\end{theorem}
the gap can be quantified as well. However, we may need to obtain an upper bound instead of a lower bound.


\section{Total variation distance} 
\cite{kieferComputingTotalVariation2018}.


\cite{desharnaisMetricsLabelledMarkov2004}
 

==> archieved/archieved-gradient-step.tex <==

\newpage 

\color{blue}
Using the method of Lagrangian multiplier, we can formulate the following unconstrained max-min problem 

$$
\mbox{maximize}_{\pi\in \Pi} \mbox{minimize}_{\mu} V(s_0, \pi) +\mu  \Expect_{\pi}\left[  B (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\right]
$$
where $\pi$ is the primal variable and $\mu$ is the dual variable. 



Based on the randomized optimization method, we use the sample approximation of the expectation value: Let $N$ be the number of sampled trajectories in the \ac{mdp} $M$, we have
\begin{align}
 &	\Expect_{\pi}\left[  B (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\right]\\
= & \sum_{y}   P(y|M^\pi) \left[  B (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\right]
\end{align}

It is observed that the randomized optimization reduces the problem into a constrained optimization where the expectation in the constraint depends on the decision variable---the policy $\pi$. Next, we discuss how to employ stochastic optimization with decision-dependent distribution \cite{drusvyatskiyStochasticOptimizationDecisionDependent2023} to approximately solve the optimization problem.

\subsection{Policy Gradient Methods for Detection-Aware Planning}

We develop an  algorithm inspired by several conceptual algorithms in stochastic optimization with decision-dependent distributions. In particular, we adopt the proximal point method for stochastic optimization which has shown to be more stable empirically. For a fixed dual variable $\mu$, the proximal point method alternates between two steps (in our context):
\begin{align*} 
\text{Proximal point: } \theta_{t+1}= \arg\min_{\theta} \mathcal{L}(\theta, P(M^{\theta_{t}}))+ \frac{1}{2\eta_t}\norm{\theta-\theta_t}^2 \label{eq:proximal-point} 
\end{align*}
where $\eta_t >0$ is a user-specified step size



Let policy $\pi$ is parameterized by $\theta$ and write the stochastic process $M^\pi$ as $M^\theta$. 
Taking the gradient with respect to policy parameter $\theta$, we have 

\begin{align}
	&  \nabla \sum_y P(y|M^\theta) \left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon)\right]\\
	= &  \sum_y  \left( \nabla  P(y|M^\theta) \cdot \left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon)\right]+P(y|M^\theta) \cdot \nabla \left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon)\right]
	\right) \\
	= &  \sum_{y\in U} \left( \nabla  P(y|M^\theta) \cdot \left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon)\right] + P(y|M^\theta) \cdot \nabla \left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)}  - \epsilon)\right]\right)\\
	= &\underbrace{  \sum_{y\in U} P(y|M^\theta)  \nabla \log  P(y|M^\theta) \cdot \left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon)\right]  }_{\text{part A}}  + \underbrace{ \sum_{y\in U} P(y|M^\theta)\nabla \left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon)\right]}_{\text{part B}}\\
 =& \sum_{y\in U} P(y|M^\theta ) (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon +1)  \nabla \log  P(y|M^\theta)
	\label{eq:last-step}
	\end{align}
where $U = \{y\in Y\mid \log\frac{P(y|M^\theta)}{P(y \mid M_0)} > \epsilon \}$.

\begin{align}
	& \nabla \log P(y|M^\theta) \\
	= &  \frac{1}{P(y|M^\theta)} \cdot\left(  \sum_{\rho \in \plays(M)} 
	P(y|\rho)	\frac{\partial  P(\rho | M^{\theta})}{\partial \theta}\right). \\
	= & \sum_{\rho \in \plays(M)}   \frac{1}{P(y|M^\theta)} \cdot P(y|\rho) P(\rho|M^\theta) 	\frac{\partial \log  P(\rho | M^{\theta})}{\partial \theta} \label{eq:partial-log-P}
  \end{align}
  where $P(y|\rho)=\obs(y|\rho)$ is the probability of receiving observation $y$ given the path $\rho$. This probability does not depend on the policy.

 Substituting \eqref{eq:partial-log-P} into the equation \eqref{eq:last-step}, 
\begin{align*} & \sum_{y\in U} P(y|M^\theta ) (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon +1)  \nabla \log  P(y|M^\theta)\\
= & \sum_{y\in U}  (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon +1) \cdot \left(\sum_{\rho \in \plays(M)}  P(y|\rho) P(\rho|M^\theta) 	\frac{\partial \log  P(\rho | M^{\theta})}{\partial \theta} \right) \\
= & \sum_{y\in U}  (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon +1) \cdot \left(\Expect_{\rho} \left[ P(y|\rho)   	\frac{\partial \log  P(\rho | M^{\theta})}{\partial \theta} \right] \right)
\end{align*}

 

 We use sampling to estimate the gradient with the following basic steps: Deterministic observation case.

 \begin{enumerate}
     \item Draw $Z=\{\rho_1,\rho_2,\ldots \rho_N\}$ samples of trajectories in $M^\theta$;
     \item For each $\rho_i$, determine its observation $y_i$ and evaluate if $y_i \in U$. Let $y_1,y_2,\ldots, y_K\in U$ for $K$ different observations in $U$ obtained from the sampled paths.
     \item For each $y_j$, $j=1,\ldots, K$,  compute $\frac{\partial \log  P(\rho_k | M^{\theta})}{\partial \theta}$ for all $\rho_k$ such that $P(y_j|\rho_k)=1$, then sum up the gradients. 
     And  multiply the sum with $(\log\frac{P(y_i|M^\theta)}{P(y_i \mid M_0)} - \epsilon +1)$. This is the term $z_j$ for observation $y_j$.
     \item the gradient is $\sum_{j=1}^K z_j$.
 \end{enumerate}


 Alternatively, we consider to use stochastic gradient descent:
\begin{align*}
& \nabla \sum_{y}   P(y|M^\pi) \left[  B (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\right]\\
  = & \nabla  \sum_{y \in \textcolor{blue}{U}}   P(y|M^\pi) (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\\
  = &   \sum_{y \in \textcolor{blue}{U}}   P(y|M^\pi) \nabla (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\\
   = &   \sum_{y \in \textcolor{blue}{U}}   P(y|M^\pi) \nabla  \log P(y|M^\pi)\\
 \approx &    \sum_{y_i \in \textcolor{magenta}{\overline U}}  \mathbf{1}(y_i=y, \rho_i=\rho) \frac{\partial \log  P(\rho | M^{\theta})}{\partial \theta} 
\end{align*} 
\textcolor{blue}
\begin{align}
	& \nabla \log P(y|M^\theta) \\
	= &  \frac{1}{P(y|M^\theta)} \cdot\left(  \sum_{\rho \in \plays(M)} 
	\obs(y|\rho)	\frac{\partial  P(\rho | M^{\theta})}{\partial \theta}\right). \\
	= & \sum_{\rho \in \plays(M)}   \frac{1}{P(y|M^\theta)} \cdot \obs(y|\rho) P(\rho|M^\theta) 	\frac{\partial \log  P(\rho | M^{\theta})}{\partial \theta}\\
	= & \sum_{\rho \in \plays(M)} \frac{ P(y,\rho|M^\theta)}{P(y|M^\theta)} \frac{\partial \log  P(\rho | M^{\theta})}{\partial \theta} \\
	\approx &    \frac{\sum  \mathbf{1}(y_i=y, \rho_i=\rho)}{ \sum \mathbf{1}(y_i=y)}   \frac{\partial \log  P(\rho | M^{\theta})}{\partial \theta} 
\end{align}
Because $\log P(\rho | M^{\theta})$ is equivalent to 
\begin{equation*}
	\log P(\rho | M^{\theta}) = \log \prod_{t=0}^{\abs{\rho}} P(s_t, a_t, s_{t+1})\pi(s_t, a_t) = \sum_{t=0}^{\abs{\rho}} \log (P(s_t, a_t, s_{t+1}) + \pi_\theta(s_t, a_t)).
\end{equation*}
Thus, $\frac{\partial \log P(\rho | M^{\theta})}{\partial \theta} = \frac{\partial \sum_{t} (\log P(s_t, a_t, s_{t+1}) + \log \pi_\theta(s_t, a_t))}{\partial \theta} = \sum_{t}\frac{\partial \pi_\theta(s_t, a_t)}{\partial \theta}\frac{1}{\pi_\theta(s_t, a_t)}$. 
\newpage 

%In part A, we can use the sample estimation of the gradient, let $y_1,y_2,\ldots, y_N$ be the observations of the sampled trajectories $\rho_1,\rho_2,\ldots, \rho_N$, 
%\begin{align*}
%\mbox{\eqref{eq:last-step}}=\frac{1}{\abs{\overline{U}}} \sum_{y_i \in \overline U}  \nabla \log  P(y_i|M^\theta) \cdot \left[  B (\log\frac{P(y_i|M^\theta)}{P(y_i \mid M_0)} - \epsilon)\right]    
%\end{align*}
%where $\overline{U} =  \{y_i \mid B (\log\frac{P(y_i|M^\theta)}{P(y_i\mid M_0)} - \epsilon)\ne 0 \}$.
\todo[inline]{The following are derivation steps, can be archived for future references. not in the main equation.}
\jf{haoxiang: This is different from the gradient you used, which only contains the second part.}

 
Noting $\nabla \log P(y_i|M^\theta) = \frac{1}{P(y_i|M^\theta)} \nabla P(y_i|M^\theta)$, the Part A can be rewrite as 
 
 
 \begin{align} 
 	& \sum_{y\in U} P(y|M^\theta)  \frac{1}{P(y_i|M^\theta)} \nabla P(y_i|M^\theta) \cdot \left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon)\right] \\
 \approx & \frac{1}{\abs{\bar U}} \sum_{y\in \bar U} \frac{1}{P(y_i|M^\theta)}
 \nabla P(y_i|M^\theta) \cdot
  \left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon)\right].\\
  = & \frac{1}{\abs{\bar U}}\sum_{y\in \bar U} \nabla \log P(y_i|M^\theta) \cdot
  \left[  \log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon\right].
 \end{align}
 where $\bar U =\{y_i \mid\left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon)\right] = \log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon \}$ is a subset of samples for which the constraint $ \log\frac{P(y|M^\theta)}{P(y \mid M_0)} \le \epsilon$ is violated under the current policy.
 
 For part B, the sample approximation is 
 \begin{align}
 	\text{Part B}  & =  \frac{1}{\abs{\bar U}} \sum_{y\in \bar U} \nabla \left[  B (\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon)\right] \\
 	&  = \frac{1}{\abs{\bar U}} \sum_{y\in \bar U}\nabla  \log P(y|M^\theta).
 \end{align}

 
 Let's combine Part A and Part B
 \begin{align}
 	\text{Part A} + \text{Part B} = \frac{1}{\abs{\bar U}} \sum_{y\in \bar U} 
 	\nabla  \log P(y|M^\theta) \cdot \left(
 	\log\frac{P(y|M^\theta)}{P(y \mid M_0)} - \epsilon +1
 	\right)
 \end{align}

Thus, we need to  calculate $\nabla \log P(y|M^\theta)$ as follows.

\begin{align}
 & 	\nabla \log P(y|M^\theta) \\
 & =  \nabla \log \sum_{\rho } P(\rho |M^\theta)\obs(y|\rho)  \\
 & =  \nabla \log \sum_{\rho } P(\rho |M^\theta)\obs(y|\rho) \\
 & =  \nabla  \prod_{\rho } \log P(\rho |M^\theta)\obs(y|\rho)\\
 & =\sum_{\rho} \prod_{\rho', \rho'\ne \rho } \log P(\rho' |M^\theta)\obs(y|\rho')\cdot   \obs(y|\rho) \nabla \log P(\rho|M^\theta) 
\end{align}
 
 Alternatively, 	we can compute the gradient as follows:
 
 \begin{align}
 	 & \nabla \log P(y|M^\theta) \\
 	= &  \frac{1}{P(y|M^\theta)} \nabla P(y|M^\theta) \label{eq:observation-gradient}
 \end{align}
    
To calculate $\frac{\partial P(y|M^\theta)}{\partial \theta}$. It is noted that different path $\rho$ may generate the same observation $y$.
\added{Given a deterministic observation function}, $P(y|M^\theta) = \sum_{\rho \in \plays(M), \obs(\rho)=y} P(\rho| M^\theta)$. As a result, 
\[
\frac{\partial P(y|M^\theta)}{\partial \theta} =\sum_{\rho \in \plays(M), \obs(\rho)=y} 
\frac{\partial  P(\rho | M^{\theta})}{\partial \theta}
\]
\jf{Haoxiang, please check the above partial derivative. it is different from the one you calculated. }

Given a probabilistic observation function, $P(y|M^\theta) = \sum_{\rho \in \plays(M)} \obs(y\mid \rho ) P(\rho| M^\theta)$. Because $\obs(y |\rho)$ is independent from $\theta$, we have 

\begin{equation}
	\label{eq:observation-gradient-2}
\frac{\partial P(y|M^\theta)}{\partial \theta} =\sum_{\rho \in \plays(M)} 
\obs(y|\rho)	\frac{\partial  P(\rho | M^{\theta})}{\partial \theta}.
\end{equation}
Note that the deterministic observation function is a special case of the probabilistic observation function.

Substituting in \eqref{eq:observation-gradient} with \eqref{eq:observation-gradient-2}


\begin{align}
	& \nabla \log P(y|M^\theta) \\
	= &  \frac{1}{P(y|M^\theta)} \cdot\left(  \sum_{\rho \in \plays(M)} 
	\obs(y|\rho)	\frac{\partial  P(\rho | M^{\theta})}{\partial \theta}\right). \\
	= & \sum_{\rho \in \plays(M)}   \frac{1}{P(y|M^\theta)} \cdot \obs(y|\rho) P(\rho|M^\theta) 	\frac{\partial \log  P(\rho | M^{\theta})}{\partial \theta}\\
	= & \sum_{\rho \in \plays(M)} \frac{ P(y,\rho|M^\theta)}{P(y|M^\theta)} \frac{\partial \log  P(\rho | M^{\theta})}{\partial \theta} \\
	\approx &    \frac{\sum  \mathbf{1}(y_i=y, \rho_i=\rho)}{ \sum \mathbf{1}(y_i=y)}   \frac{\partial \log  P(\rho | M^{\theta})}{\partial \theta} 
\end{align} 
Then term $ \frac{\partial \log P(\rho | M^{\theta})}{\partial \theta}$, $\log P(\rho | M^{\theta})$ is equivalent to 
\begin{equation*}
	\log P(\rho | M^{\theta}) = \log \prod_{t=0}^{\abs{\rho}} P(s_t, a_t, s_{t+1})\pi(s_t, a_t) = \sum_{t=0}^{\abs{\rho}} \log (P(s_t, a_t, s_{t+1}) + \pi_\theta(s_t, a_t))
\end{equation*}
\textcolor{red}{Thus $\frac{\partial \log P(\rho | M^{\pi})}{\partial \pi} = \frac{\partial \sum_{t} (\log P(s_t, a_t, s_{t+1}) + \log \pi(s_t, a_t))}{\partial \pi} = \sum_{t}\frac{\partial \pi(s_t, a_t)}{\partial \pi}\frac{1}{\pi(s_t, a_t)}$.}
\jf{Haoxiang, take a look at policy gradient method and see how to calculate the policy gradient with respect to policy function parameter $\theta$ and revise the above expression for the partial derivative of the policy with respect to $\theta$. }
 

\newpage
\jf{The following is the previous draft.}

 
Assume $N$ trajectories $\rho$ are generated, for each trajectory $\rho_i$, we have the corresponding $y_i$. then $\Expect_{\pi}\left[  B (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\right] =\sum_{i = 1}^N\left[  B (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\right]$   Let $g(\pi) = \sum_{i = 1}^N\left[  B (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\right]$. Calculating the derivate of $g(\pi)$ with respect to $\pi$ is 
\[
\frac{\partial g(\pi)}{\partial \pi} = \frac{1}{N}\sum_{i = 1}^N\frac{\partial}{\partial \pi}(\log\frac{P(y_i|M^\pi)}{P(y_i \mid M_0)} - \epsilon)
\]
where $\log\frac{P(y_i|M^\pi)}{P(y_i \mid M_0)} - \epsilon > 0$. If $\log\frac{P(y_i|M^\pi)}{P(y_i \mid M_0)} - \epsilon \le 0$, then $B (\log\frac{P(y_i|M^\pi)}{P(y_i \mid M_0)} - \epsilon) = 0$, whose derivative is $0$ with respect to $\pi$. Thus we only consider the $y$ which $\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon > 0$. Assume the $y$ satisfying the above condition consists of a set $U$. Based on the above analysis, we have
\[
\frac{\partial g(\pi)}{\partial \pi} = \frac{1}{N}\sum_{y \in U}\frac{\partial}{\partial \pi}(\log P(y|M^\pi)) = \frac{1}{N}\sum_{y \in U}\frac{1}{P(y|M^\pi)}\frac{\partial P(y|M^\pi)}{\partial \pi}
\]
Next, we calculate $\frac{\partial P(y|M^\pi)}{\partial \pi}$. It is noted that different $\rho$ may generate the same $y$. So 
\[
\frac{\partial P(y|M^\pi)}{\partial \pi} = \sum_{\text{obs}(\rho) = y}\frac{\partial P(Y = y|\rho, M^{\pi})P(\rho | M^{\pi})}{\partial \pi}
\]
Since $P(Y = y|\rho, M^{\pi})$ is independent of the policy $\pi$, so the above equation is equivalent to 
\[
\frac{\partial P(y|M^\pi)}{\partial \pi} = \sum_{\text{obs}(\rho) = y}P(Y = y|\rho, M^{\pi}) \frac{\partial P(\rho | M^{\pi})}{\partial \pi}
\]
$\frac{\partial P(\rho | M^{\pi})}{\partial \pi}$ can be written as $P(\rho | M^{\pi}) \frac{\partial \log P(\rho | M^{\pi})}{\partial \pi}$, $\log P(\rho | M^{\pi})$ is equivalent to 
\[
\log P(\rho | M^{\pi}) = \log \Pi_{t} P(s_t, a_t, s_{t+1})\pi(s_t, a_t) = \sum_{t} \log (P(s_t, a_t, s_{t+1}) + \pi(s_t, a_t))
\]
Thus $\frac{\partial \log P(\rho | M^{\pi})}{\partial \pi} = \frac{\partial \sum_{t} (\log P(s_t, a_t, s_{t+1}) + \log \pi(s_t, a_t))}{\partial \pi} = \sum_{t}\frac{\partial \pi(s_t, a_t)}{\partial \pi}\frac{1}{\pi(s_t, a_t)}$.

So far, we have 
\[
\frac{\partial g(\pi)}{\partial \pi} = \frac{1}{N}\sum_{y\in U} \sum_{\text{obs}(\rho) = y}\frac{P(Y = \text{obs}(\rho)| \rho, M^{\pi})}{P(\text{obs}(\rho))| M^{\pi})}P(\rho|M^{\pi})(\sum_{t}\frac{1}{\pi(s_t, a_t)}\frac{\partial \pi(s_t, a_t)}{\partial \pi})
\]

Considering the derivative of $V(s_0, \pi)$ with respect to $\pi$. Use the sampling-based method. Assume $N$ trajectories $\rho$ are generated. Then the value $V(s_0, \pi)$ can be estimated as $\sum_{i = 1}^NR(\rho_i)$, based on the policy gradient method, $\frac{\partial V(s_0, \pi)}{\partial \pi} = \frac{1}{N}\sum_{i = 1}^N\left((\sum_{t = 0}^{T-1}\frac{\partial \log(\pi(s_t, a_t))}{\partial \pi})(\sum_{t = 0}^{T-1} \gamma^{t}r(s_t, a_t)) \right)$.

Let $L(\pi, \mu) = V(s_0, \pi) +\mu  \Expect_{\pi}\left[  B (\log\frac{P(y|M^\pi)}{P(y \mid M_0)} - \epsilon)\right]$, we have $\frac{\partial L(\pi, \mu)}{\partial \pi} = \frac{\partial V(s_0, \pi)}{\partial \pi} + \mu \frac{\partial g(\pi)}{\pi}$.

==> archieved/archieved-problem1.tex <==

 
\begin{comment}
 \begin{problem}
 	Given a \ac{mdp} $M$ without the reward function, a partial observation function $\obs$,  a set $\mathcal{ X} = \{0, 1,2,\ldots, N\}$ of \emph{reference HMMs}  generated from $M$ based on a set of reference policies. For each $ i\in {\cal X}$, the reference policy $\pi_i$ is optimal with respect to a reward function $R_i$. Assuming the agent's reward function is $R_0$. 
 	Compute a policy $\pi$ in $M$ that maximizes the total  (discounted) reward w.r.t. $R_0$ while ensuring the probability of a correct guess made by the passive observer about the agent's reward is less than $\xi$.
 \end{problem}

 

\begin{definition}[The guessing function]
	Let $X$ be a set of hypotheses, $Y$ be the set of observations, The MAP rule-based guessing function is $\kappa: Y \rightarrow \mathcal{X}$ such that 
	\[
	\kappa(y) = \max_{x\in \mathcal{X}} P(X=x \mid Y=y).
	\]
	where the posterior probability is computed from the reference HMMs.
\end{definition}


\begin{definition}
	Given a distribution over observations $P_Y$,  the probability of not choosing $0\in \mathcal{X} $ made by the MAP estimator is 
	\begin{multline} P(\mbox{Not choose } 0 ) = \sum_{y\in \mathcal{Y}}P(\arg\max_{x\in \mathcal{X}}P(X=x|Y=y) \ne 0)P_Y(y)\\
	=\sum_{y\in \mathcal{Y}} \mathbf{1} (\underline{p}> P(X= 0 |Y=y)) P_Y(y). 
\end{multline}
	where $\underline{p} = \min_{x\in \mathcal{X} \setminus \{0\}} P(X=x|Y=y)$.
\end{definition}
 

\begin{definition}[Vulnerable observations  against a Naive observer]
An observation $y\in Y$    is \emph{vulnerable} agaist a Naive observer for the objective $0$ if and only if the following conditions are satisfied:
$$
\min_{x\in \mathcal{X}\setminus \{0\}} P(X=x | Y=y) <  P(X=0 | Y=y).
$$
\end{definition}


\begin{remark}
    Alternatively, we can consider a generalized likelihood ratio test to have the opponent uses EM to learn about a HMM from the observation and use that HMM for generalized likelihood ratio test (GLRT). Using the second method, we can determine a set of \emph{safe} observations against a strong observer who employs GLRT.
\end{remark}
\begin{definition}[safe observations against a strong observer]
    An observation $y\in Y$    is \emph{safe} against a strong observer for the objective $ 0$ if and only if the following conditions are satisfied:
$$
\log\frac{P(Y=y |x^\ast(y) )}{P(Y=y| X= 0)} < \epsilon $$
where $\epsilon$ is determined from the significance level $\alpha$ and $x^\ast(y)$ is the maximum likelihood estimate given the observation $y$. 
\end{definition}

In other words, if the null hypothesis is $0$, then by observing a safe observation $y$ and the observer performing a generalized likelihood ratio test, that observer won't reject the null hypothesis. The GLRT does not assume/use the information of alternative hypotheses.

Based on this definition, we define a vuleranble observation for a given intention. 

\begin{definition}{Vulnerable observations against a strong opponent}
    Given a set $\mathcal{X} $ of  hypotheses with $0$ being the true intention, an observation is vulnerable for $0$ if and only if all the other alternative hypotheses are rejected \added{but not the hypothesis $0$}. In other words, we have 

$$
\log  \frac{P(Y=y| x^\ast(y))}{P(Y=y| X = x)}> \epsilon, \forall x\in \mathcal{X}\setminus \{0\}
.$$

\added{
$$
\log  \frac{P(Y=y| x^\ast(y))}{P(Y=y| X = 0 )} < \epsilon,  
.$$}
\end{definition}
The vulnerability property is based on the idea of eliminating alternatives using generalized likelihood ratio test.

\jf{We can remove the second condition to construct a superset of vulnerable observations.}

To determine if an observation is vulnerable given the strong observer case, the ML estimate of the HMM given observation $y$ is required. However, this computation can be expensive. 

Since the planner knows the ground truth policy employed, the following result can be derived.

\begin{lemma}
    Let $\pi$ be a policy employed by the planning agent and $x$ is the true intention, we say that the policy is \emph{vulnerable} with probability $\le \alpha$ if the following condition is satisfied:

\begin{equation}
\label{eq:vulnerable-policy}
\sum_{y\in \mathcal{Y}}\Pr (Y=y\mid M^\pi) \mathbf{1}(\min_{x\in  \mathcal{X}\setminus \{0\}} \log\frac{P(Y=y|x^\ast(y))}{P(Y=y \mid X =x)} > \epsilon) <\alpha.
\end{equation}

\end{lemma}

In the case that $\calX =\{0,1\}$ that include only two hypotheses, \eqref{eq:vulnerable-policy} can be expressed as 

\begin{equation}
\label{eq:vulnerable-policy}
\sum_{y\in \mathcal{Y}}\Pr (Y=y\mid M^\pi) \bm{1}(  \log\frac{P(Y=y|x^\ast(y))}{P(Y=y \mid M_0)} > \epsilon) <\alpha.
\end{equation}


Since the true distribution of observations is generated by the agent with policy $\pi$, thus, the best estimate the opponent can obtain is $M^\pi$. Then we can replace the maximum likelihood estimate $x^\ast(y)$ by the ground truth $M^\pi$ and formulate a constrained optimization problem for planning subject to constraints on the vulnerability.
\begin{problem}
The optimal planning problem can be formulated as follows:
\begin{align}
\label{eq:deception-planning}
    &\max_\pi V_0(s_0, \pi)\\
   &  \text{subject to: } \\
   & \sum_{y\in \mathcal{Y}}\Pr (Y=y\mid M^\pi) \bm{1}(  \log\frac{P(Y=y|M^\pi)}{P(Y=y \mid M_0)} > \epsilon) <\alpha.
\end{align}
\end{problem}

This problem is not the same as 
\begin{align}
\label{eq:kl-constrained}
    &\max_\pi V_0(s_0, \pi)\\
   &  \text{subject to: } \\
   & \sum_{y\in \mathcal{Y}}\Pr (Y=y\mid M^\pi)  \log\frac{P(Y=y|M^\pi)}{P(Y=y \mid M_0)}) <\eta.
\end{align}

\jf{can we relate the two problems?}


 A heuristic approach:
\begin{itemize}
    \item Start with some policy $\pi^0$. Let $k=0$.
    \item At iteration $k$, use the HMM under $\pi^k$ and the alternative hypothesis $1$ to compute a set of vulnerable observations:

    $$Y_v^k=  \{y\mid  \log\frac{P(Y=y|M^{\pi^k})}{P(Y=y \mid M_0)} > \epsilon \} $$
    \item Update the policy $\pi^k$ to $\pi^{k+1}$ to avoid the vulnerable observations with high probability $1-\alpha$ while maximizing the total reward.
    \item Repeat 2-3 until convergence (measured by 1) the vulnerable observations becomes a subset of previous vulnerable observations and 2) the value under the policy converges.)
\end{itemize}

Hypothesis: The algorithm converges if the set of vulnerable observations in the $k$-th iteration is a superset of the vulnerable observations in the $k-1$-th iteration. 
\end{comment}


==> archieved/archieved_hmm_pdfa.tex <==


\newpage It is also proven in \cite{dupontLinksProbabilisticAutomata2005} that for each HMM, one can find an equivalent \ac{pnfa} with no final probabilities. The \ac{pnfa} is a tuple 
\[
A = \langle  {\cal X} , O, \delta, s_0, \tau \rangle 
\]
where the transition function $\delta: {\cal X}\times O\times {\cal X} \rightarrow [0,1]
$ is defined such that $\delta(x, o,x') =  \emission(o|x) \trans(x,x') $. The function $\tau: {\cal X } \rightarrow [0,1]$ is a mapping defining the final probability of each state. In this setting, $\tau(x)=0$ for all $x\in {\cal X}$.

The \ac{pnfa} can be nondeterministic because it is possible that for the same state $x$ and the same observation $o$, both $\delta(x,o,x_1)>0$ and $\delta(x,o,x_2)>0$ yet $x_1\ne x_2$. To see this, consider that the policy $\pi_0$ is a randomized one, then from a given state, say $s$, $\pi_0(s,a)=\pi_0(s,b)=0.5$, then the corresponding transitions in the \ac{pnfa} are $\delta (s,\obs(s), (s,a))=0.5$ and $\delta (s,\obs(s), (s,b))=0.5$ where $(s,a),(s,b)$ are different states in the \ac{pnfa}. 

\jf{first, an \ac{pnfa} can be approximated by \ac{pdfa} of exponential size (prefix-tree structure).Second, if the observation set is a finite, then there always exists a \ac{pdfa} to express the same distributions. however, pdfa may not need to be involved at all. To see how \ac{pnfa} can be transformed into \ac{pdfa}, the notions of suffix distributions and $\mu$-distinguishability are needed.}

\begin{definition}[Suffix distributions]
    Let $\rho \in O^\ast$ be a finite observation sequence, called a \emph{prefix}, the \emph{suffix distribution} of $\rho$ is defined by 
    \[
    \gamma(\rho' \mid \rho) =\frac{ \Pr(\rho \rho') }{\Pr(\rho O^\ast)}
    \]
    where $\Pr(\rho O^\ast)$ is the probability of observing $\rho$, followed by any observation sequence.
\end{definition}

\begin{definition}[$\mu$-Distinguishability \cite{clarkPAClearnabilityProbabilisticDeterministic2004}]
For $\mu>0$, two prefixes $\rho_1,\rho_2$ are \emph{$\mu$-distinguishble} if $L_\infty(\gamma(\rho_1)-\gamma(\rho_2)) >\mu$. That is, there exists a \emph{distinguishing suffix} $\rho$ such that $\abs{\gamma(\rho_1\rho) - \gamma(\rho_2\rho )} \ge \mu$. 
\end{definition}
Question: is $\mu$-distinguishability define a relation: If $\rho_1,\rho_2$ are $\mu$-indistinguishable, and $\rho_2, \rho_3$ are $\mu$-indistinguishable, will it be possible that $\rho_1,\rho_3$ are $\mu$-distinguishble?
The answer is NO.

\paragraph*{Determinizing PNFA to PDFA: Finite support case}

Given a \ac{pnfa} over finite support, there always exists a \ac{pdfa} that defines the same distribution.  See Guttman's thesis p. 39 for the construction. 

\paragraph*{Prefix tree with bounded length $L$} The root of the tree is a unique symbol $\lambda$, referred to as an empty string. The tree is generated recursively as follows: From the root $\lambda$, for each $\sigma \in \Sigma$, a labeled directed edge $\lambda \xrightarrow{\sigma}\sigma$ is defined and $\sigma$ is a child of $\lambda$. 
Let $w\in \Sigma^k$ where $k< L$ be a node in the tree, which is represented as a word of length $k$, for each $\sigma \in \Sigma$, a labeled directed edge $w\xrightarrow{\sigma} w\sigma $ is included; a node $w\in \Sigma^\ast$ with length $L$ is a leaf. The construction repeats until a leaf is reached.

The prefix tree automaton $\cal T$ gives a structure of a PDFA. Given an \ac{pnfa} $\cal A$ that describes a distribution over $\Sigma^\ast$, the truncated distribution over $\Sigma^L$ can be obtained from the \ac{pnfa} and denoted by $\Pr_{\cal A}$

The states of the \ac{pdfa} is the set of nodes in the prefix tree automaton. For $w$ denoting one of the state/node, for an edge $w \xrightarrow{\sigma} w\sigma$, we set the transition probability 
\[
P_A(w,\sigma, w\sigma) = \frac{\sum_{x\in \Sigma^\ast}  \Pr_{\cal A}(w \sigma x)}{\sum_{x\in \Sigma^\ast} \Pr_{\cal A}(wx)}
\]

\jf{Question: How to compute the probability $\Pr_{\cal A}$ for any word $w$ given the truncated distribution over $\Sigma^L$?}


Once the \ac{pdfa} is constructed, we can then aggregates states that are $\mu$-indistinguishable, so that the size of the \ac{pdfa} can be minimized. The horizon length $L$ may be selected.

\begin{remark}
On page 56 of Guttman's thesis, he mentioned that the distribution of a PFA can be approximated using the distribution generated by a PDFA with exponentially size. He pointed towards another thesis Zeitouni 1992.
\end{remark}

% The \ac{pdfa} can be constructed from the \ac{pnfa} as follows:
% \begin{itemize}
% \item $\hat Q$ is a finite set of states, each state $\hat q $ corresponds to a sequence of   inputs of the original \ac{pnfa}. Let $R: \hat Q\rightarrow (Q\times \Sigma)^\ast Q$ be such a mapping. 
% \item The initial state is $\lambda$
% \item The transition function is defined as follows: Consider $\hat q_1$, $R(\hat q_1) = (o_0o_1\ldots o_n)$, given an input $o$, if $\delta(\hat q_1, o, \hat q_2)=p$ where $p= \Pr(o\mid o_0o_1\ldots o_n)$, and $R(\hat q_2)= R(\hat q_1)\circ o$.
% \end{itemize}
% \begin{definition}[Prefix-tree automata]
% Given a \ac{pnfa} $A= (Q,O,\delta, \iota) $ (without terminating probability) and an integer $n$, a probability distribution $P$ over $O^n$ is defined such that for any $\rho \le O^n$,
% \[
% P(\rho) = \sum_{ q, q' \in Q} \iota(q) \delta(q, \rho,q'); 
% \]
% Here the summation is due to nondeterministic transitions, an input word $\rho$ may have different runs reaching different states.

% Because $O^n$ is a finite set, given $P$, for each $\rho \in O^n$, we can define its suffix distribution using the definition. Two prefixes $\rho_1,\rho_2$ can be merged if their suffix distributions are $\mu$-indistinguishable. 



    
\end{definition}

==> convergence_analysis.tex <==
\subsection{Convergence analysis}

The policy gradient of the Langrangian 
can be rewritten into the following:
\begin{multline*}
\nabla_\theta L^\beta(\theta, \lambda) = 
\nabla_\theta V(s_0, \theta) 
- \beta \nabla_\theta D_{KL}(P_{\theta_t} ||P_\theta) - 
 \lambda \nabla_\theta C (s_0, \theta) 
\end{multline*}
where $C(s_0,\theta) = \sum_{x\in X} w_{ x,\theta} \nabla_\theta P_\theta(x)$. Here, the parameters $w_{ x,\theta}\ge 0$ for all $x\in X$ can be viewed as a weight associated with each trajectory. Specifically, the weight $w_{x,\theta} =  \sum_{y\in U} P(y|x) $ is understood as the probability of generating an observation $y$ that violating the detection constraint. Recall the definition of $U = \{y\in \mathcal{Y} \mid  \log\frac{P( y; M_\theta)}{P( y; M_0)} - \epsilon \ge 0\}$. The dependency of the weights on the policy parameter $\theta$ is manifested in the dependency of the set $U$ on the policy parameter $\theta.$

If the weights are independent from the policy parameter $\theta$, then the primal gradient ascent is generic proximal policy gradient with the value function $\tilde V = V(s_0,\theta) - \lambda C(s_0,\theta)$. 


[Closeness of two policies means the constraint can be satisfied.]
Given two policies $\pi_{\theta_1}$ and $\pi_{\theta_2}$, if $D_{KL}(P_{\theta_t} ||P_\theta) \le \epsilon$ and  $\Pr \left( \log\frac{P(Y;M_{\theta_1})}{P(Y;  M_0)}   
 \ge  \epsilon    ; M_{\theta_1} \right) \le \alpha. $ then 
 \[
\Pr \left( \log\frac{P(Y;M_{\theta_2})}{P(Y;  M_0)}   
 \ge  \epsilon    ; M_{\theta_2} \right) \le \alpha.
 \]
 







==> images/mdp-thm1-nominal.tex <==
\trimbox{0cm 0cm 0cm 0cm}{ 
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto, scale=0.7,transform shape]

  \node[state,initial] (0) {$0$};
  \node[state] (1) [right of=0] {$1$};
  \node[state] (2) [above right of=0] {$2$}; 
  \path [->](0) edge              node {$H$} (1)
        (0) edge              node {$T$} (2)
        (1) edge   [loop right]          node {$H$} (1)
        (1) edge              node {$T$} (2)
        (2) edge   [bend left]           node {$H$} (1)
        (2) edge  [loop right]            node {$T$} (2);
\end{tikzpicture}
}


==> images/mdp-thm1-user0.tex <==
\trimbox{0cm 0cm 0cm 0cm}{ 
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto, scale=0.7,transform shape]
  \node[state,initial] (0) {$0$};
  \node[state] (1) [right of=0] {$1$};
  \node[state] (2) [above right of=0] {$2$}; 
  \path [->](0) edge              node {$0.5$} (1)
        (0) edge              node {$0.5$} (2)
        (1) edge   [loop right]          node {$0.5$} (1)
        (1) edge              node {$0.5$} (2)
        (2) edge   [bend left]           node {$0.5$} (1)
        (2) edge  [loop right]            node {$0.5$} (2);
\end{tikzpicture}
}

==> images/mdp_proof.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto, scale=0.7,transform shape]

  \node[state,initial] (1) {$1$};
  \node[state] (2) [above of=1] {$2$};
  \path [->](1) edge   [loop below]          node {$H$} (1)
        (1) edge              node {$T$} (2)
        (2) edge   [bend left]           node {$H, 0.5$} (1)
        (2) edge   [loop left]           node {$H, 0.5$} (2)
        (2) edge  [loop right]            node {$T$} (2);
\end{tikzpicture}


==> main-v3.tex <==
\section{Augmented Lagrangian}


==> oldProof.tex <==
\begin{proof}
    \begin{figure}[htbp]
        \centering     
        \begin{subfigure}[c]{0.2\textwidth}
        \input{images/mdp-thm1-nominal}
        \caption{}
        \label{fig:mdp}
        \end{subfigure}
        \begin{subfigure}[c]{0.2\textwidth}
         \input{images/mdp-thm1-user0}
        \caption{}
        \label{fig:nominal}
        \end{subfigure}
        \caption{The \ac{mdp} and the Markov chain induced by the nominal policy}
        \label{fig:mdp-mc}
    \end{figure}

    We prove this theorem by constructing such a case. Consider a simple   \ac{mdp} with $S= \{0,1,2\}$ and deterministic transitions $P(1|0,H)=1$, $P(2|0, T)=1$, $P(1|1,H)=1$, $P(2|1,T)=1$, $P(1|2,H)=1$ and $P(2|2,T)=1$, illustrated in Fig.~\ref{fig:mdp}.
An agent is allowed to take $N$ actions and then terminated.    The nominal hypothesis is that at each state, the user  selects ``H'' or ``T'' with equal probabilities. The Markov chain induced by this nominal user's policy is shown in Fig.~\ref{fig:mdp-mc}.
The observer can observe the states but not the actions. It is not hard to see that the stochastic process induced by the nominal policy describes the sequence  of outcomes for flipping a fair coin for $N$ times where state 1 means a head is observed in the last flip and 2 means a tail is observed in the last flip.
    

The reward function for the planning agent is $R(s,H)=1$ and $R(s,T)=0$ for every $s\in S$. Therefore, if the agent is to maximizes the total discounted reward, it would select only action ``H'' at every state to maximize the total discounted rewards. 

Consider the observer employs a hypothesis testing: With a confidence level $\alpha$ and total $N$ of coin flips, the observer would reject the nominal hypothesis $M_0$ if either the number of heads or the number of tails is greater than or equals an integer $K$. For example, if $\alpha=0.05$, $N=10$, then the null hypothesis $M_0$ is rejected if the heads is less than 2 or greater than 8.


Then, a policy that obtains the maximal total discounted reward without being $(1-\alpha)$-covert can be computed from the following \ac{mdp} whose state variable is augmented with two counters, one  keeping  track of the number of times action ``H'' is selected and the other keeping track of the number of times action ``
T'' is selected. That is $\bar M= (\bar S, A, \bar P)$ such that $\bar P((s',k+1,\ell)|(s,k,\ell),H)=1$ and $\bar P((s'',k,\ell+1)|(s,k,\ell),T)=1$ provided that $P(s'|s,H)$ and $P(s''|s,T)$ are defined in the original \ac{mdp} and $k+\ell \le N$. If $k+\ell =N$, then $\bar P(\sink \mid (s, k, \ell), H ) = \bar P(\sink \mid (s, k, \ell), T )=1$, where $\sink$ is a unique sink state.

With this finite memory, the agent can take $H$ with the constraint that the total number of ``H'' or the total number of ``tails''
never exceeds $K$---ensuring the $(1-\alpha)$-covertness and maximizes the total  reward as a constrained \ac{mdp} in $\bar M$. Let $\pi^\ast$ be the finite-memory optimal policy. The total reward obtained by this finite-memory policy is $\frac{(1-\gamma^{K-1})}{1-\gamma}$.

Next, we can formulate a constrained \ac{mdp} in the original \ac{mdp} 

\begin{align}
    & \max_{\vec{m}} \sum_{s\in S} m(s,H)R(s, H)\\
    \text{subject to: } &\sum_{s\in S} m (s, a) = \gamma \sum_{s'\in S, a'\in A} P(s|s',a')m(s',a')+\mu(s'), \\
     & \forall s\in S, \nonumber 
\end{align}
\begin{align}
   & \vec{m}\succeq 0, \\
    & \sum_{s\in S} m(s, H) \le \frac{K-1}{N},
\end{align}
where $m(s,a)$ is the discounted probability of reaching state $s$ and taking action $a$ under the constrained optimal policy.

We select $\gamma = 0.95$, given $\alpha = 0.05$, $N = 10$, and $K = 8$, the total reward obtained by the finite-memory policy is $\frac{1-0.95^7}{1-0.95} = 6.03$. By solving the constrained \ac{mdp}, the total reward obtained by a Markov policy is $0.7$. Thus we conclude no Markov policy that ensures to obtain a total reward greater than $K-1$ and ensures with a probability less than $\alpha$, the number of heads or the number of tails is smaller than $K$ in total of $N$ flips. 
\end{proof}

\jf{the solution for the Markov policy is incorrect. here is the corrected proof}

\color{blue}
Next, we construct a Markov policy in the original \ac{mdp} using the augmented \ac{mdp} $\bar M$. 


\begin{align}
    & \max_{\vec{m}} \sum_{s\in S} m(s,k, \ell, H)R(s, km \ell, H)\\
    \text{subject to: } &\sum_{(s,k,\ell)} m (s,k, \ell, a) =  \sum_{(s',k',\ell'),  a'\in A} P(s|s',k', \ell', a')m(s',k', \ell' , a')+\mu(s',k', \ell'), \\
     & \forall s\in S, \nonumber \\
   & \vec{m}\succeq 0, \\
    & \frac{\sum_{s, k, \ell} m(s,k, \ell, H)}{\sum_{s, k, \ell} (m(s,k, \ell, H)+ m(s,k,\ell, T))} \le \frac{K-1}{N},\\
    & \frac{m(s, k, \ell, H)}{(m(s,k, \ell, H)+ m(s,k,\ell, T))= \frac{m(s, k', \ell', H)}{(m(s,k', \ell', H)+ m(s,k',\ell', T))}, \forall k,k', \ell, \ell'.
\end{align}
\todo[inline]{the equation is incomplete.}
The last constraint enforces that the policy does not depend on the number of heads or tails that has been selected in the past.  

\normalcolor

==> subsections/approximation.tex <==
\subsection{Approximation through state-merging}


==> subsections/hmm.tex <==

\paragraph{Information structure} 

PO: the grey agent, with a nominal behavior/reward funciton $R_0$.


P1: the planning agent, with a reward function $R_1$. 

P2: the observer.

\begin{definition}[Observation function] The state -observation function of P2 is $\obs_S : S  \rightarrow \dist{O}$ that maps a state $s$ to a distribution $\obs(s)$ over observations. The action observation function is state dependent, defined as $\obs_A: S\times A \rightarrow \dist{O}$ that maps an action $a$ from $s$ to a distribution $\obs_A(s,a)$ over observations. 
\end{definition}
Without loss of generality, we write $\obs: S\cup S\times A\rightarrow \dist{O}$ the combined   state and action observation function.

Note that in traditional POMDP, because the planning agent is the one who makes action decisions, the action is always observed. This is not the case when the planning agent is different from the observer. Therefore, the state observation function follows from the general POMDP definition and we need to specify the action observation function. The action observation function is in general state dependent. For example, one action $a$ may be invisible when the state is $s$ but becomes observable when the state is $s'$. Action invisible and action visible POMDP are both special cases.
\jf{todo, this action visible/invisible POMDP is not defined.}

The following information structure is considered:
\begin{itemize}
\item P1 has perfect observations.
\item P2 has partial observation, defined by $\obs$.
\item P2 knows that the nominal user has perfect observations.
\end{itemize}

Under this information structure, we can assume a nominal, Markovian policy $\pi_0: S\rightarrow \dist{A}$   for the user. Under this nominal policy $\pi_0$, P2's observation stochastic process can be described using an \ac{hmm}. 

\begin{definition}[HMM modeling P2's observation given the nominal policy $\pi_0$]
Given the \ac{mdp} $M =(S,A, P, s_0)$, the nominal policy $\pi_0: S\rightarrow \dist{A}$, and an observation function $\obs:S\cup S\times A\rightarrow \dist{O}$, the stochastic process of observations is captured using a discrete HMM(with state emission), 
\[
HMM  = \langle {\cal X}, O, \trans, \emission, s_0 \rangle 
\]
 \begin{itemize}
    \item ${\cal X} = S \cup S\times A$, including two types of states, a decision state $s$ at which an action will be selected, and a nature's state $(s,a)$ at which the next state will be determined according to a probability distribution.  
    \item  $  O$ is an alphabet, the set of observations;
    \item  $\trans: {\cal X}  \times {\cal X}\rightarrow[0,1]$ is the mapping defining the probability of each transition. The following constraints are satisfied: For $s\in S$, 
    \[
\trans (s, (s,a))= \pi_0(s, a );
    \]
    For $(s,a)\in S\times A$, 
    \[
\trans( (s,a),s' ) =  P( s,a, s');
    \]
    \item $\emission: {\cal X} \times O \rightarrow [0,1]$ is a mapping defining the emission probability of observation at state that satisfies the following constraints:
    \[
    \emission(  s,o )  =\obs(o\mid s),
    \]
    and 
    \[
    \emission(  (s,a),o ) = \obs(o\mid s,a).
    \]
 \end{itemize}    
\end{definition}
It can be validated that the HMM is well-defined. 


Next, we formulate a probabilistic planning problem for nonrevealing intention deception strategy against partially observable P1. We first restrict the planning horizon to be upper bounded by an integer $T$. 

\begin{definition}[Finite-horizion intention-deception planning]

\[
\mathcal{M} = 
\langle X, A, \mathcal{P}, \mathcal{R} ,x_0 \rangle 
\]
where 
\begin{itemize}
\item $X\coloneqq S\times O^{\le T}\times [0,\varepsilon]$ is the finite state space, where $S$ is the discrete state space of the original \ac{mdp}, $O^{\le T}$ is a finite set of observations up to length $T$, $\varepsilon$ is the threshold for detection.
\item The transition function is defined as follows. For a given state $x=(s, \rho, c)$, if $\rho\in O^{\le T-2}$ and $c\le \varepsilon$, then for any action $a\in A$, let 
\[
\mathcal{P}(x, a, (s', \rho 
 \circ o_1 \circ o_2, c')) = P(s,a,s') \obs((s,a),o_1)\obs(s',o_2),
\]
where $\circ$ is the operator for concatenation and the observation $\rho$ is concatenated with the new observations $o_1,o_2$ of the last action played and the resulting state. 

And the last component $c$ is updated to $c'$ as follows:
\[
c ' =\begin{cases}
 c -  \ln\frac{ \obs((s,a), o_1)\obs(s',o_2) }{\Pr_0(o_1o_2 \mid \rho)} & \text{ if } c -  \ln\frac{ \obs((s,a), o_1)\obs(s',o_2) }{\Pr_0(o_1o_2 \mid \rho)} >0 \\
 0 &\text{ otherwise.}
 \end{cases}
 \] 
in which the term $\Pr_0(\obs(s,a)\obs(s') \mid \rho)$ is the probability of receiving these new observation given the \ac{hmm} of the user's policy. Such a probability can be computed using the forward algorithm \url{https://web.stanford.edu/~jurafsky/slp3/A.pdf}.

 
 In words, the transition probability consists of two components. One is determined by the HMM, which is the probability of generating observation $\rho'$ given the observation $\rho$ and the action $a$. Another one is the cost, which is calculated via the cost update formula given the action $a$ and the new observation $\rho'$.\jf{HX: PLEASE ADD EXPLANATION.}

On the other hand, if $\rho \in O^T$ or $c \ge \varepsilon$, then the state $(s,\rho, a)$ becomes a sink state.
\item The reward function $R$ is defined as follows. Given $x = (s, \rho, c)$, the reward function is:
\begin{equation*}
     R(x, a) =  \left\{
    \begin{array}{ll}
    r(s, a) & \text{ if }  c \neq 0,\\
    0 & \text{ if } c = 0.
\end{array}\right.
\end{equation*}
where $r(s, a)$ is the reward function of the attacker's MDP.
\jf{HX:COMPLETE the definition of the reward function.}
\item $x_0 $ is the initial state distribution. $P(x_0 =(s_0,o_0, c_0)) = \obs(s_0,o_0)$ where $c_0=0$. This is because the initial state  $s_0$ is the same for both nominal user and the attacker. 
\end{itemize}
\end{definition}


Given a state-action sequence $\rho= s_0a_0s_1a_1\ldots s_n $, a \ac{hmm} $HMM_\rho$ can be constructed as follows.
\[
HMM_\rho= \langle  O, \calX_\rho, \mathbf{P}_\rho, \mathbf{E}, s_0\rangle 
\]
where $\calX_\rho =  \{s_i,i=0,\ldots, n\} \cup \{(s_i,a_i), i=0,\ldots, n-1\}$, $\mathbf{P}_\rho: \calX_\rho \times \calX_\rho \rightarrow[0,1]$ is the mapping definition the probability of each transition and satisfying the following constraints: For each $s_i$, $\mathbf{P}_\rho(s_i,(s_i,a)) =1$ if $a=a_i$ and   $\mathbf{P}_\rho(s_i,(s_i,a)) =0$
otherwise.
The emission probability is the same as in $HMM_0$.

Consider a finite horizon of observations $n$, 
let $S^k_n$ be the log-likelihood ratio between the null hypothesis, \ie, \ac{hmm} $HMM_0$, and the alternative hypothesis, \ac{hmm} $HMM_\rho$ constructed for a state-action sequence $\rho=s_0a_0s_1\ldots s_n$, 
\[
S_n^k = \log (\prod_{i=k}^n \gamma_i) = \log (\prod_{i=k}^n \frac{\Pr_\rho(O_i\mid O_{0}^{i-1})}{\Pr_0(O_i\mid O_{0}^{i-1})}) = \sum_{i=k}^n \log \frac{\Pr_\rho(O_i\mid O_{0}^{i-1})}{\Pr_0(O_i\mid O_{0}^{i-1})}, \quad k\le n 
\]
where $O_{0}^K$ is the finite observation from step $0$ to step $K$. 


From this relation, the cost $c$ is indeed the loglikelihood ratio  between  the observations given alternative hypothesis $HMM_\rho$, generated by a deterministic state-action sequence (what actually occured), and the observations given the null hypothesis $HMM_0$. 

\begin{definition}[The value of intention deception]
Considering the attacker plans without intention deception, the expected reward for the attacker to obtain is $r_0$. When the attacker plans with intention deception, the expected reward for the attacker to obtain is $r_i$. Then the value of intention deception is $r_i - r_0$.
\jf{How do you define this quantity?}
\end{definition} 

 \begin{theorem}
 \jf{main message. what the solution provides us.}
 \end{theorem}
\begin{proof}
todo
\end{proof}


